Self-Supervised Domain Adaptation for Visual Navigation with Global Map Consistency

We propose a light-weight, self-supervised adaptation for a visual navigation agent to generalize to unseen environment. Given an embodied agent trained in a noiseless environment, our objective is to transfer the agent to a noisy environment where actuation and odometry sensor noise is present. Our method encourages the agent to maximize the consistency between the global maps generated at different time steps in a round-trip trajectory. The proposed task is completely self-supervised, not requiring any supervision from ground-truth pose data or explicit noise model. In addition, optimization of the task objective is extremely light-weight, as training terminates within a few minutes on a commodity GPU. Our experiments show that the proposed task helps the agent to successfully transfer to new, noisy environments. The transferred agent exhibits improved localization and mapping accuracy, further leading to enhanced performance in downstream visual navigation tasks. Moreover, we demonstrate test-time adaptation with our self-supervised task to show its potential applicability in real-world deployment.

==> 3_method.tex <==
\section{Method}
We introduce a simple and generic, self-supervised learning method for noise-robust visual navigation. 
Our objective is to transfer a pre\-trained agent to novel, unseen environments where different types of actuation and odometry sensor noises are present. 
The proposed method enforces consistency on global maps  generated over time in a round-trip trajectory. 
In this section, we explain the overall setup, the various types of actuation and sensor noise and how the global map consistency is implemented. We also introduce our data augmentation method. 
\paragraph{Problem Setup} 
The embodied agent receives a RGB observation, $o_{t}$ and an odometry sensor measurement, $s_{t}$.         
At each step, the model, $f_\theta$, predicts the pose, $p_{t}$ and a global occupancy grid map, $M_{t}$. $\theta$ is the trainable parameters
and the pose, $p_{t}$, is represented as  $(x, y, \phi)$ where $x$ and $y$ denote the 2D pose coordinate and $\phi$ indicates the 1D orientation.  
\begin{equation}
    f_{\theta}(o_{1:t},s_{1:t}) = p_{t}, M_{t}
\end{equation}
The agent outputs an action, $a_{t}$ by the policy, $\pi_{\psi}$. $\psi$ is the pre\-trained policy parameters.  
\begin{equation}
    \pi_{\psi}(M_{t},p_{t}) = a_{t}
\end{equation}
The agent executes a discrete action from the following action space: \{ Forward, Right, Left \}.
Note that our proposed task is applicable to most visual navigation agent based on spatial map memory. 
Furthermore, we replicate realistic actuation and odometry noise models~\cite{Chattopadhyay2021RobustNavTB} to demonstrate the feasibility of the self-supervised learning in more complex, novel environments. 

\paragraph{Actuation and Odometry Sensor Noise} 
The properties of actuation noise fall into two classes; motion bias, and motion drift. 
First, the motion bias adds a constant bias, $\delta_{c} \in \mathbb{R}^{3}$, and a stochastic bias, $\delta_{s} \in \mathbb{R}^{3}$ drawn from $ \mathcal{N}(\mu_s,\Sigma_{s})$.
Then, the motion drift, $\alpha \in \mathbb{R}^{3}$, is added towards left or right only for the forward movement. 
The actuation noise is the addition of both motion bias and motion drift. 
\begin{equation}
    \epsilon_{act} = \delta_{c} + \delta_{s} + \alpha 
\end{equation}
The ground-truth pose of the agent after an action is defined as 
\begin{equation}
    (x_{t+1},y_{t+1},\phi_{t+1}) = (x_{t}, y_{t}, \phi_{t}) + (u_x,u_y,u_\phi) + \epsilon_{act}
\end{equation}
where the $(u_x,u_y,u_\phi)$ indicates the intended action control. 

In addition, the pose reading noise from odometry sensors are drawn from a Gaussian Mixture model.
The final pose reading is measured as 
\begin{equation}
   (x_{t+1}',y_{t+1}',\phi_{t+1}') = (x_{t+1},y_{t+1},\phi_{t+1}) + k \epsilon_{sen}
\end{equation}
where k denotes the sensor noise severity. 
\paragraph{Global Map Consistency}
Our agent learns to generalize across various noise models through the global map consistency. 
The pose estimation error accumulates over time since both actuation noise and odometry sensor noise are statistically independent for each measurement. 
This leads to embedding more accurate pose data in the global map generated in the earlier steps compared to the ones generated later in a continuing trajectory. 

To implement the self-supervised learning task efficiently, we drive an embodied agent in round-trip trajectories. 
The round-trip is easily generated by executing any navigational task for a designated number of steps, turning around 180\textdegree, and executing the previous action sequence in reverse. 
In a noiseless setting, the agent observes the same area at each one-way trip.  
Therefore, the global map from its forward path should be equal to the global map generated during its backward path.
We learn from this consistency. 

When the actuation noise is present, the agent may not step on the same way\-points it has traversed during its forward path. Nonetheless, our proposed formulation is still valid as the agent generates maps from overlapping area. 

To summarize, during the forward path, the agent generates a reference global map, $M_{\text{ref}}$. 
\begin{equation}
    f_{\theta}(o_{1:t_r},s_{1:t_r}) = p_{t_r}, M_{\text{ref}}  
\end{equation}

where $t_{r}$ is the step after the robot turns around.
On its way back, the agent generates a new map, but continues the pose estimation based on its last estimated pose. 
The same global coordinate is shared across all global maps. 
At each reverse step, a new global map, $M_{t}$, is predicted. 
\begin{equation}
    f_{\theta}(o_{t_r+1:t},s_{1:t}) = p_{t}, M_{t} 
\end{equation}

Lastly, our self-supervised task use the MSE loss to impose the consistency between the predicted $M_{t}$ and $M_{\text{ref}}$. In the equation below, T denotes the ending point of the trajectory and $\mathtt{stopgrad}$ indicates that no back\-propagation should happen through $M_{\text{ref}}$.
\begin{equation}
    \mathcal{L} = \sum_{t=t_r+1}^{T}\|\mathtt{stopgrad}(M_{\text{ref}}) - M_t\|_{2}
\end{equation}

\paragraph{Data Augmentation}
We introduce a data augmentation method based on random cropping which has been used in various type of data such as videos or images.~\cite{takahashi2019data, hansen2020self}. In a trajectory, we randomly sample three time\-steps in a chronological order ; the initial point, the half-way point, and the ending point. Indicating each point as $p_{i}$, $p_{h}$, and $p_{e}$, our loss formulation is defined as 
\begin{equation}
\begin{split}
    \mathcal{L} =\sum_{t=t_{h}+1}^{t_{e}}\|\mathtt{stopgrad}(f_{\theta}&(o_{t_i:t_h},s_{t_i:t_h})) \\
    & - f_{\theta}(o_{t_h+1:t},s_{1:t})\|_{2}
\end{split}
\end{equation}
We demonstrate the enhancement of learning performance using data augmentation in the experiment section. 
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{./Figures/task_overview.png}
\end{center}
   \caption{Task Overview}
\label{fig:long}
\label{fig:onecol}
\end{figure}
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%

%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{./Figures/data_augmentation.png}
\end{center}
   \caption{Data Augmentation}
\label{fig:long}
\label{fig:onecol}
\end{figure}
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%



==> 3_method_v2.tex <==
3956\section{Method}


We introduce a simple and generic, self-supervised learning method for noise-robust visual navigation. 
Our objective is to transfer a pre\-trained agent to novel, unseen environments where different types of actuation and odometry sensor noises are present. 
The proposed method enforces consistency on global maps  generated over time in a round-trip trajectory. 
In this section, we explain the overall setup, the various types of actuation and sensor noise and how the global map consistency is implemented. We also introduce our data augmentation method. 


\subsection{Visual Navigation with Spatial Memory}

Our self-supervision works on the consistency of the global map, therefore can be applied to most visual navigation agents that are based on spatial map memory~\cite{karkus2021differentiable, chaplot2020learning, chaplot2020object, wani2020multion,zhang2017neural,ramakrishnan2020occupancy}. 
Such approaches  train two neural networks for mapping and planning, which we will refer as $f_\theta$ and $\pi_\psi$ respectively.

The mapping module $f_\theta$ predicts a global map $M_t$ and the pose $p_{t}$ given the observation $o_t$ and the odometry sensor measurement $s_t$,
\begin{equation}
f_{\theta}(o_{1:t},s_{1:t}) = M_{t}, p_{t}.
\end{equation}
For the purpose of proposition, we demonstrate the applicability using a sequence of RGB image observations for $o_t$ as the input, and the 2D occupancy grid map for $M_t$ and the 2D pose for $p_t=(x,y,\phi)$.
Here $(x,y)$ denote the 2D coordinate and $\phi$ indicates the 1D orientation.

Then the planning module $\pi_\psi$ is implemented with a separate neural network, which is a policy network that observes the output of the mapping module and generates the action $a_t \in \mathcal{A}$
\begin{equation}
    \pi_{\psi}(M_{t},p_{t}) = a_{t}.
\end{equation}
We allow a discrete set of agent actions, specifically $\mathcal{A}$=\{Forward, Right, Left\}.

Our supervision works on the intermediate representation between the two modules, namely the consistency of $M_t$.
Note that the consistency of $M_t$ is tightly coupled with the accuracy of $p_t$ because the pose $p_t$ can be defined with respect to the generated map $M_t$ and the network $f_\theta$ fuses the current observation to $M_t$ using the current pose $p_t$.
The formulation allows to disentangle the variations in measurements from the policies designed for different downstream tasks. 
We can train a desired policy network $\pi_\psi$ in an ideal simulation set-up with the ground truth oracle and fine-tune only the observation module $f_\theta$ in a different environment set-up.



\paragraph{Actuation and Odometry Sensor Noise} 
We first train both networks in a noiseless set-up and demonstrate the feasibility of the proposed self-supervision in realistic  noise models.
There are two main streams of expected variation; actuation and sensor noise.
Large amount of both classical and latest work~\cite{khosla1989categorization, gonccalves2008sensor, habitat19iccv} has presented the approach to model realistic actuation and odometry noise. 
In this section, we briefly describe the noise models used as an unseen environment for the trained agent.
An exhaustive discussion is available in ~\cite{Chattopadhyay2021RobustNavTB}.

The actuation noise disturbs an agent's movement. 
The agent fails to reach the intended position, and it becomes difficult to estimate the agent's pose solely by the control commands.
The properties of actuation noise fall into two classes; motion bias, and motion drift. 
First, the motion bias adds a constant bias, $\delta_{c} \in \mathbb{R}^{3}$, and a stochastic bias, $\delta_{s} \in \mathbb{R}^{3}$ drawn from $ \mathcal{N}(\mu_s,\Sigma_{s})$.
Then, the motion drift, $\alpha \in \mathbb{R}^{3}$, is added towards left or right only for the forward movement. 
The actuation noise is the addition of both motion bias and motion drift
\begin{equation}
    \epsilon_{act} = \delta_{c} + \delta_{s} + \alpha. 
\end{equation}
The ground-truth pose of the agent after an action is defined as 
\begin{equation}
    (x_{t+1},y_{t+1},\phi_{t+1}) = (x_{t}, y_{t}, \phi_{t}) + (u_x,u_y,u_\phi) + \epsilon_{act},
    \label{eq:pose_actuation_noise}
\end{equation}
where the $(u_x,u_y,u_\phi)$ indicates the intended action control. 

In addition, the odometry sensor noise affects the pose estimation accuracy, which further degrades the mapping accuracy and the navigation performance.
The pose reading noise from odometry sensors are drawn from a Gaussian Mixture model.
The final pose reading is measured as 
\begin{equation}
   (x_{t+1}',y_{t+1}',\phi_{t+1}') = (x_{t+1},y_{t+1},\phi_{t+1}) + k \epsilon_{sen},
   \label{eq:pose_odometry_noise}
\end{equation}
where the $k$ denotes the sensor noise severity.
The noise models are derived from the real-world observation, and we employ them based on the noise parameters obtained from actual physical deployment to test the performance of our algorithm in noisy environment.

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{./Figures/fig2.png}
\end{center}
   \caption{Task Overview}
\label{fig:long}
\label{fig:onecol}
\end{figure}
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%
\subsection{Self Supervision with Global Map Consistency}
\label{sec:self-supervision}

We assume deploying an pre-trained agent in an unseen environment, where the ground truth poses or the changes in the observation noise model is not known.
Instead, we can create a supervision signal by enforcing consistency of the generated global map $M_t$.
While we cannot assure that the map is error-free, we can assume that the error accumulates over time.
This leads to incorporating more accurate pose data in generating the global map in the earlier steps compared to the ones generated later in a continuing trajectory. 

To implement the self-supervised learning task efficiently, we deliberately design overlapping trajectories and drive an embodied agent in round trips. 
The round trip is easily generated by executing any navigational task for a designated number of steps, turning around 180\textdegree, and executing the previous action sequence in reverse. 
The global map is first generated during the forward path, then the agent resets and generate another map from scratch during the backward path.
In a noiseless setting, the agent observes the same area at each one-way trip.  
Therefore, the global map from its forward path should be equal to the global map generated during its backward path.
When the actuation noise is present, the agent may not step on the same way\-points it has traversed during its forward path. Nonetheless, our proposed formulation is still valid as the agent generates maps from overlapping area. 

To summarize, during the forward path, the agent generates a reference global map $M_{F}$
\begin{equation}
    f_{\theta}(o_{1:t_r},s_{1:t_r}) = M_{F}, p_{F}, 
\end{equation}
%
where $t_{r}$ is the step when the robot turns around.g
On its way back, the agent generates a new map.   
However, the same global coordinate is shared across all global maps and the agent maintains the estimated poses and continues incremental pose estimation using the full odometry $s_{1:t}$.
At each reverse step, a new global map, $M_{B,t}$, is predicted,
\begin{equation}
    f_{\theta}(o_{t_r+1:t},s_{1:t}) = M_{B,t}, p_{B,t},\quad t>t_r.
\end{equation}

Lastly, our self-supervised task imposes the consistency between the predicted $M_{F}$ and $M_{B,t}$ to fine-tune the mapping module $f_\theta$ under new environment. 
In the equation below, T denotes the ending point of the trajectory and $\mathtt{stopgrad}$ indicates that no back\-propagation should happen through $M_{F}$
\begin{equation}
    \mathcal{L} = \sum_{t=t_r+1}^{T}\|\mathtt{stopgrad}(M_{F}) - M_{B,t}\|_{2}.
    \label{eq:consistency}
\end{equation}
Therefore we compare the estimated map at every step during the backward path, providing a rich set for loss computations per acquired trajectory.
While there are several ways of finding the difference between the two binary maps, we incorporated the mean squared error (MSE) loss. 
The choice of losses is further discussed in the experiment section.

%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
\includegraphics[width=1.0\linewidth]{./Figures/fig3.png}
\end{center}
   \caption{Data Augmentation}
\label{fig:long}
\label{fig:onecol}
\end{figure}
%%%%%%%%% Replace Figure %%%%%%%%%%%%%%%%%%%%


\paragraph{Data Augmentation}
While our vanilla formulation utilize the bisections of round-trip trajectories, the consistency can be enforced for any subsets of trajectories with overlapping observations.
We introduce a data augmentation method based on random cropping which has been used in various types of data such as videos or images.~\cite{takahashi2019data, hansen2020self}.
Given a trajectory, we randomly sample three time\-steps in a chronological order: the initial point $t_1$, the half-way point $t_o$, and the ending point $t_2$ $(t_1 < t_o < t_2)$. 
Then the reference map ${M}_F'$ is produced from  $f_{\theta}(o_{t_1:t_o},s_{t_1:t_o})$ and compared to the map ${M}_{B,t}'$ generated from the backward step $f_{\theta}(o_{t_o+1:t},s_{1:t})$, $t_o<t<t_2$.
Our loss formulation is defined as 
\begin{equation}
    \mathcal{L} =\sum_{t=t_{o}+1}^{t_{2}}\|\mathtt{stopgrad}({M}'_F)  - {M}'_{B,t}\|_{2}.
\end{equation}
We demonstrate the performance enhancement using data augmentation in the experiment section. 




==> 4_experiments.tex <==
\section{Experiments}
We extensively evaluate our self-supervised learning task to provide answers to the following questions. 
i. Does the proposed task enhance the pose estimation, mapping and navigation task performance? 
iii. Can the proposed task train agents to generalize across various environments? 
iii. Can we utilize the task for test-time deployment? 

\subsection{Experiment Setup}
We use the Habitat~\cite{habitat19iccv} simulator which enables training embodied agents in interactive 3D environments for various tasks. 
Habitat embeds photo-realistic 3D scans of the real indoor environments. We experiment in the scenes from Gibson dataset~\cite{xia2018gibson} and analyze on the standard train/val/test split~\cite{savva2019habitat}. 
The main odometry and actuation noise model in our experiments is based on real data collected from Locobot ~\cite{chaplot2020learning}. % reference Locobot
We evaluate if our self-supervised learning task can enhance the agent’s performance in pose estimation and mapping. 
We report the translation and rotation errors in median values and MSE loss for the occupancy grid map accuracy.
To evaluate the performance of navigational agents, we implement the agent trained for exploration from ~\cite{chaplot2020learning} and follow the task setup proposed by ~\cite{chen2019learning}. 
We show our result for exploration since it becomes the fundamental task for most navigation agents.
The agent is trained to maximize the area coverage within a designated number of steps, which is 1000 steps in all of our experiments. 
After each episode, the agent reports two metrics; the absolute coverage area in $m^2$ and the ratio of area coverage.  
Therefore, in our setup, we train an agent in a noiseless environment where the pose and map estimator, $f_{\theta}$, is trained with the ground-truth pose and egocentric map.  
We then observe if our proposed approach can help the agent to generalize across various environments without ground-truth supervision. 
We implement our task using PyTorch~\cite{paszke2019pytorch}. 
The training time of the following experiments, accelerated with a RTX 1080 GPU, completes within 5 minutes and the test-time adaptation finishes in 2.5 minutes. 
Additional training details are available in the supplementary material. 
 
\subsection{Baselines}
Throughout the experiments, our model, which is trained with self-supervised learning task, is compared against two baselines. 
The first baseline is the model trained in a noiseless environment with ground-truth information.
The model demonstrates the performance of the agent pre-trained in a noiseless simulator and immediately deployed in a new, noisy environment.
Thus, the model before adaptation sets the lower\-bound in evaluating if our proposed adaptation method successfully leads to performance enhancement. 
Furthermore, we provide an upper\-bound baseline.  
The pre-trained model is fine-tuned with ground-truth supervision in the new environment. The performance of the fine-tuned model shows the target performance for our adaptation model. 
However, note that it is difficult to fine-tune a model in the real world since the ground-truth pose information is not available. 
To summarize, we denote the pre-trained model as "No Adaptation" and the model fine-tuned with the ground truth data as "GT Train" in our result. 
Our self-supervised learning approach aims at training the "No Adaptation" models to generalize for the new noise and environment, and become comparable to the "GT Train" model. 


\subsection{Results}
\paragraph{Generalization to noisy environments}
We first observe if our proposed self-supervised learning task helps agents to transfer to a new, noisy environment. 
Given a pre-trained agent in a noiseless environment, we assess the pose estimation, mapping and navigation task performance of our agent trained with self-supervised learning.
The number reported in Table ** demonstrates the performance enhancement in all evaluations.  
In addition to the enhancement in pose estimation, the agent successfully generates occupancy representation as accurate as the GT Trained agent does. 
Furthermore, our agent learns to better perceive the surroundings and explores 91.79\% of its environment when tested for exploration. 
Our agent distinctively outperforms the baseline agent which is immediately deployed without adaptation.
The qualitative result is also shown in **. 


\begin{table}[]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lccc}
      \toprule 
      \textbf{} & \textbf{} & \textbf{No Adaptation} & \textbf{GT Trained} & \textbf{Ours}\\
      \midrule 
      \multirow{2}{*}{Pose} & x,y (m) & 0.15 & 0.02 & 0.03 \\
                                & theta (deg) & 2.67 & 0.27 & 0.36 \\
      \midrule
      \text{Mapping} & MSE loss & 0.25 & 0.17 & 0.17\\
      \midrule
      \multirow{2}{*}{Exploration} & Ratio(\%) & 82.02 & 93.75 & 91.79\\
                & Area($m^2$) & 26.36 & 31.83 & 30.79\\
      \bottomrule 
\end{tabular} 
}
\end{center}
  \caption{Generalization to noisy environments}
\end{table}

\paragraph{Task Robustness to Odometry Noise Increase}
While the previous experiment demonstrates that an agent can transfer to a noisy environment, we also experiment to see if the proposed task can transfer agents to various noise conditions.
As explained in section 3.1, we set up six environments where the sensor noise severity, k, in equation 4 ranges from 0 to 5. 
We immediately test the pre-trained model in the new environments. 
Nonetheless, our agent is separately trained in each environment with the self-supervised learning task. The agent trained with ground-truth supervision is also trained at each environment for fair comparison. In plot **, we see that our self-supervised agent consistently reports superior performance against the agent which is not fine-tuned. The result guarantees that the proposed self-supervised learning task can be utilized for various agents regardless of its odometry sensor noise level. 

\paragraph{Task Robustness to Acutation Noise Increase}

We further address the task’s applicability in environments with changing values of actuation noise properties. 
We observe if the pre\-trained agent stably transfers to the new noise-added environments. 
In the new environment, we add the actuation noise model from Locobot.
To variate the properties of actuation noise more specifically, we also combine a noise model, similarly proposed in ~\cite{Chattopadhyay2021RobustNavTB}.
We add a constant motion bias and stochastic motion bias, sampled at each step. 
For every forward movement, motion drift value is also added to the noise. 
Our final noise model thus creates a more challenging environment for agents. 
The result is reported in **. 
In all cases, our transferred agent shows superior performance against the pre-trained model and exhibits high performance on a par with the GT Train model. 


\begin{table}[]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lccc}
      \toprule 
      \textbf{} & \textbf{} & \textbf{No Adaptation} & \textbf{GT Trained} & \textbf{Ours}\\
      \midrule 
      \multirow{2}{2cm}{Constant Motion Bias} & \text{x,y(m)} & 0.16 & 0.03 & 0.04\\
         & \text{theta(\textdegree)} & 2.69 & 0.28 & 0.3\\
      \midrule
      \multirow{2}{2cm}{Stochastic Motion Bias} & \text{x,y(m)} & 0.16 & 0.04 & 0.05\\
         & \text{theta(\textdegree)} & 2.77 & 0.32 & 0.34\\
      \midrule
      \multirow{2}{2cm}{Motion Drift} & \text{x,y(m)} & 0.18 & 0.05 & 0.06\\
         & \text{theta(\textdegree)} & 3.91 & 0.49 & 0.82\\
      \bottomrule 
\end{tabular} 
}
\end{center}
  \caption{Robustness to Actuation Noise}
\end{table}

\paragraph{Task Robustness to Path Length}
We analyze if our proposed method is trainable regardless of trajectory path length. 
We assess whether the largely accumulated pose error for longer trajectories impedes agents from training with the self-supervised learning task. 
Our experiment evaluates the adaptation performance when an agent learns from trajectories at different length, varying from 100 steps up to 600. 
In each case, the pre\-trained agent first collects trajectories of designated number of steps in a new, noisy environment. 
Next, the agent learns from each set of collected trajectories with the proposed self-supervised learning task.  
As the step length increases with 100 steps interval, we observe diminishing enhancement as shown in plot $()$. 
Nonetheless, our proposed method still noticeably exceeds the lower bound performance across various trajectory lengths. 

\paragraph{Test-Time Adaptation}
For test-time adaptation, we investigate the scenario where the agent is trained and tested in a validation environment with new actuation and odometry noise. 
We collect 20 trajectories for training and test the agent’s performance on 80 trajectories both within the same environment. 
The experiment is designed to demonstrate the task’s applicability for real\-world deployment scenarios. 
The GT train agent is fine\-tuned in a new scene with ground\-truth data provided and tested in the same scene during 80 test trajectories. 
In table **, our agent performs highly accurate pose estimation and mapping. Moreover, in the exploration task result, our agent outperforms the GT train agent. 
During the test-time adaptation, our light-weight self-supervised learning finishes training an agent within 2.5 minutes. 
Our result guarantees that the proposed task can quickly adapt agents in a real world deployment setting. 



\begin{table}[]
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|lccc}
      \toprule 
      \textbf{} & \textbf{} & \textbf{No Adaptation} & \textbf{GT Trained} & \textbf{Ours}\\
      \midrule 
      \multirow{2}{*}{Pose} & \text{x,y(m)} & 0.15 & 0.02 & 0.05\\
        & theta(\textdegree) & 2.73 & 0.25 & 0.5\\
      \midrule
      \text{Mapping} & \text{MSE loss} & 0.16 & 0.11 & 0.12\\
      \midrule
      \multirow{2}{*}{Exploration} & \text{Ratio(\%)} & 82.02 & 91.06 & 92.25\\
        & Area($m^2$) & 26.36 & 30.65 & 31.27\\
      \bottomrule 
\end{tabular} 
}
\end{center}
  \caption{Test-Time Adaptation}
\end{table}


\subsection{Ablation study}
In this section, we study ablated versions of our self-supervised learning method. 
All experiments are conducted in the same condition, unless mentioned.

\paragraph{Data Augmentation}
Given 100 trajectories collected with the pre\-trained agent, we augment the data with the proposed random cropping method from section 3.2. 
We ablate this technique to see if the agents trained with self-supervised learning task generalize better when trained with augmented trajectories. 
In table **, we compare our agent against the agent trained without data augmentation. 
Our agent estimates the pose more accurately, showing that data augmentation helps agents to generalize across environments. 

\paragraph{Step-wise Supervision}
Our agent back-propagates the global map consistency loss at every step during the backward path. 
We examine if the step-wise supervision is necessary. In Table **, we present the result when the agent learns from the self-supervised learning only at its last step. 
As shown in Table **, we show that training the self-supervised learning task at every step exhibits more accurate pose estimation and mapping compared to the ablated agent which trains only at the last step. 

\paragraph{MSE vs. BCE Loss} 
We ablate our global map consistency loss. 
Our agent uses BCE loss in place of MSE loss for the ablation study. 
BCE loss is used in many studies for map prediction~\cite{karkus2021differentiable,chaplot2020learning} as it provides a good measurement for grid-wise classification.
BCE loss helps to train the mapper portion of the model, better classifying if each grid of a top-down map is occupied or has been explored from the agent's first perspective observation. 
BCE loss however results in poor pose estimation performance. 
Since we only train the pose estimation portion of the model during the self-supervised learning, MSE loss helps our agent to learn the distance between the predicted global map and the target map.

\begin{table}
\begin{center}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|ccc} 
\toprule
                                & \multicolumn{2}{c}{\textbf{Pose}} & \textbf{Mapping}    \\
\midrule
                            & x,y(m) & theta(deg)      & MSE error  \\
\midrule
Ours     & 0.03   & 0.36            & 0.17       \\
Ours w/o data augementation & 0.06   & 0.41            & 0.19       \\
Ours w/ last step update         & 0.15   & 2.57            & 0.24       \\
Ours (BCE Loss)             & 0.16   & 2.78            & 0.26       \\
\bottomrule
\end{tabular}
}
\end{center}
\caption{Ablation Study}
\end{table}

\paragraph{Forward vs. Backward Error}
In plot **, we also present our experiment which logs the accumulated pose estimation error during round-trip trajectories. We observe that both x,y and theta error increase for all agents as they progress in a trajectory. However, while the agent trained in a noiseless environment experience the steep increase during the backward steps, our agent consistently accumulates the pose estimation error within a similar extent during its forward and backward path. Moreover, during the turning steps at the half-way pose, the no adaptation agent experience the increase of orientation error and decrease in the position error. Although the similar trend is shown in our agent, the self-supervised learning task optimizes the agent to experience less variation.  

%%%%%%%%% TEMPORARY PLOTS %%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\columnwidth, trim = {0 2cm 0 3cm}, clip]{Figures/len_th.pdf}
\includegraphics[width=1\columnwidth,trim = {0 2cm 0 3cm}, clip]{Figures/len_xy.pdf}
\end{center}
   \caption{Path Length}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\columnwidth, trim = {0 2cm 0 3cm}, clip]{Figures/odom_th.pdf}
\includegraphics[width=1\columnwidth,trim = {0 2cm 0 3cm}, clip]{Figures/odom_xy.pdf}
\end{center}
   \caption{Robustness to Odometry Noise}
\label{fig:long}
\label{fig:onecol}
\end{figure}

\begin{figure}[t]
\begin{center}
% \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
\includegraphics[width=1\columnwidth, trim = {0 2cm 0 3cm}, clip]{Figures/fw_bw_th.pdf}
\includegraphics[width=1\columnwidth,trim = {0 2cm 0 3cm}, clip]{Figures/fw_bw_xy.pdf}
\end{center}
   \caption{Forward and Backward Path.}
\label{fig:long}
\label{fig:onecol}
\end{figure}





==> Tables/sup_table_1.tex <==

\begin{table}[]
\begin{center}
\resizebox{0.7\textwidth}{!}{%
\begin{tabular}{@{}l|ccc@{}}
\toprule
& Standard Experiment & Test-time Adaptation & Ablation Study \\ 
& (Section 4.1) & (Section 4.2) & (Section 4.3) \\
\midrule
\midrule
\multicolumn{4}{l}{\textbf{Pre-Training}} \\ 
\midrule
Dataset split & Train & Train & Train \\ \midrule
Actuation and Odometry Noise & Noiseless & Noiseless & Noiseless \\ \midrule
% Trajectory length  & 1000 & 1000 & 1000 \\ \midrule
\midrule
\multicolumn{4}{l}{\textbf{Fine-Tuning}} \\ 
\midrule
Dataset split & Train & Val & Train \\ \midrule
Actuation and odometry noise & Noisy & Noisy & Noisy  \\ \midrule
No. of trajectories & 160 & 20 & 160     \\ \midrule
Trajectory length  & 100 & 100 & 100 \\ \midrule
Training iterations & 4000 & 2000 & 4000 \\ \midrule
\midrule
\multicolumn{2}{l}{\textbf{Evaluation}} &  & \\ 
\midrule
Dataset Split  & Val & Val & Val \\ \midrule
Actuation and odometry noise & Noisy & Noisy & Noisy  \\ \midrule
No. of trajectories  & 140  & 80 & 140  \\ \midrule
Trajectory length  & 100 & 100 & 100 \\ 
\bottomrule
\end{tabular}%
}
\end{center}
\caption{Training details for standard experiment, test-time adaptation, and ablation study.}
\label{table:training_details}
\end{table}

==> Tables/sup_table_2.tex <==


\begin{table}[]
\begin{center}
\resizebox{0.25\textwidth}{!}{
\begin{tabular}{l|cc}
    \toprule 
    \multicolumn{1}{l}{Metric} & BCE & MSE \\
    \midrule
    Mean & \text{1.02e-05} & \text{3.74e-07} \\
    Max & \text{0.0044} & \text{0.0002} \\
    Variance & \text{4.18e-09} & \text{5.63e-12} \\
    \bottomrule
\end{tabular} 
}
\end{center}
\caption{Gradient Analysis on BCE and MSE}
\label{table:gradient_analysis}
\end{table}
